Exact sampling of determinantal point processes with sublinear time preprocessing

We study the complexity of sampling from a distribution over all index subsets of the set $\{1,...,n\}$ with the probability of a subset $S$ proportional to the determinant of the submatrix $\mathbf{L}_S$ of some $n\times n$ p.s.d. matrix $\mathbf{L}$, where $\mathbf{L}_S$ corresponds to the entries of $\mathbf{L}$ indexed by $S$. Known as a determinantal point process, this distribution is used in machine learning to induce diversity in subset selection. In practice, we often wish to sample multiple subsets $S$ with small expected size $k = E[|S|] \ll n$ from a very large matrix $\mathbf{L}$, so it is important to minimize the preprocessing cost of the procedure (performed once) as well as the sampling cost (performed repeatedly). For this purpose, we propose a new algorithm which, given access to $\mathbf{L}$, samples exactly from a determinantal point process while satisfying the following two properties: (1) its preprocessing cost is $n \cdot \text{poly}(k)$, i.e., sublinear in the size of $\mathbf{L}$, and (2) its sampling cost is $\text{poly}(k)$, i.e., independent of the size of $\mathbf{L}$. Prior to our results, state-of-the-art exact samplers required $O(n^3)$ preprocessing time and sampling time linear in $n$ or dependent on the spectral properties of $\mathbf{L}$. We also give a reduction which allows using our algorithm for exact sampling from cardinality constrained determinantal point processes with $n\cdot\text{poly}(k)$ time preprocessing.

==> A01_actual_implementation.tex <==
%! TEX root = neurips.tex
\section{How to compute things in practice}\label{appendix-rls}
Given a subset $\X_m$ of $m$ points from $\X$ (i.e.~$m$ rows of $\X$), let $\P$ be the projection matrix on the span of $\X_m^\transp$, i.e.
\begin{align*}
\P = \X_m^\transp(\X_m\X_m^\transp)^+\X_m = \X_{m}^\transp \L_{mm}^+ \X_m,
\end{align*}
where $\L_{mm} \in \R^{m \times m}$ is the sub-matrix of the likelihood kernel
$\L$ corresponding to $\X_m$ (i.e.~the $m$ rows and columns corresponding the $m$ sub-sampled points),
and $\L_{nm} \in \R^{n \times m}$ is a similarly defined sub-matrix with the likelihood between all $n$
points and the $m$ subsampled ones.

Then the embedding $\Z \in \R^{m \times \infty}$ is
\begin{align*}
\Z := (\selmatrix\X\X^\transp\selmatrix^\transp)^{+/2}\selmatrix\X, && \Z^\transp\Z = \P,
\end{align*}
so that for $\xbt_i = \Z\x_i$ we have $\x_i^\transp\P\x_j = \xbt_i^\transp\xbt_j$, and $\Xbt = \X\Z^\transp = \L_{nm}\L_{mm}^{+/2} \in \R^{n \times m}$.

From now on we define $\Lbh$ as
\begin{align*}
\Lbh = \X\Z^\transp\Z\X^\transp = \L_{nm}\L_{mm}^+\L_{nm}^\transp = \Xbt\Xbt^\transp,
\end{align*}
and choose $\Bh = \Xbt = \L_{nm}\L_{mm}^{+/2}$. This is also the traditional definition of Nystrom approximation.
It is easy to present, but gives little insight in terms of underlying tools used (i.e.~for that we need to introduce $\X$ and the projection).
Nonetheless if we want to explain everything in terms of $\L$ it works well enough.

Then the algorithm becomes as follow.

\textbf{Phase 1: constructing }$\DA$

We first need to compute $\Bh$, which means computing the set of $m$ points.
This is accomplished using BLESS. The main parameter in input to BLESS is $\qbar_{B}$, which should be set
to $\qbar_{B} = \cO(\log(n)/\varepsilon_B^2)$, but usually $\varepsilon_B = 1/\sqrt{2}$ and $\qbar_B \in [2,10]$ suffices. This generates
a dictionary $\DB$ with size $\cO(\qbar_{B}\deff) = \cO(\deff\log(n)/\varepsilon_B^2)$. We
then use $\DB$ to estimate RLS $\tau_i$ (note that these are not yet our $l_i$) for all $i \in [n]$.

Using $\tau_i$, we sample a new dictionary $\DA$, this time with constant $\qbar_{D} \gg \qbar_{B}$, which would
be set again to $\qbar_{D} = \cO(\log(n)/\varepsilon_D^2)$ but this time $\varepsilon_D = 1/\deff^2$.
In practice, $\qbar_{D} \in [2,10]$ seems again to suffice.
In the end we have
a dictionary $\DA$ with size $m = \cO(\qbar_{D}\deff) = \cO(\deff\log(n)/\varepsilon_D^2)$.

\textbf{Phase 2: precomputing stuff }

Using $\DA$, we can now compute $\Bh$. We also introduce $\A_{mm} = \Bh^\transp\Bh$ to act
as a $\R^{m \times m}$ counterpart to $\Lbh$. Then we compute a bunch of things as follow
\begin{align*}
l_i &= \x_i^\transp(\P\X^\transp\X\P + \I)^{-1}\x_i
= \x_i^\transp(\I - \P\X^\transp(\X\P\X^\transp + \I)^{-1}\X\P)\x_i\\
&= [\X\X^\transp - \X\P\X^\transp(\X\P\X^\transp + \I)^{-1}\X\P\X^\transp]_i\\
&= [\X\X^\transp - \Bh\Bh^\transp(\I+\Bh\Bh^\top)^{-1}\Bh\Bh^\transp]_i\\
&= [\X\X^\transp - \Bh\Bh^\transp\Bh(\I+\Bh^\top\Bh)^{-1}\Bh^\transp]_i\\
&= [\X\X^\transp - \Bh(\I + \Bh^\transp\Bh)(\I+\Bh^\top\Bh)^{-1}\Bh^\transp + \Bh(\I+\Bh^\top\Bh)^{-1}\Bh^\transp]_i\\
&= [\X\X^\transp - \Bh\Bh^\transp + \Bh(\I+\Bh^\top\Bh)^{-1}\Bh^\transp]_i\\
&= [\L - \Lbh]_i + \normsmall{(\I+\Bh^\top\Bh)^{-1/2}\Bh_i^\transp\e_i}_2^2\\
&= [\L - \Lbh]_i + \normsmall{(\I+\A_{mm})^{-1/2}\Bh_i^\transp\e_i}_2^2.
\end{align*}
Computationally, this means that we simply compute $\Bh$, and then
$[\Lbh]_i$ is the norm of the $i$-th row of $\Bh$, and $\normsmall{(\I+\Bh^\top\Bh)^{-1/2}\Bh_i^\transp\e_i}_2^2$
can be computed efficiently using a Cholesky decomposition of $\I+\A_{mm}$ and
the function \url{solve_triangular}.
To compute $\sh$ we simply sum $l_i$, to compute $\st$ we compute the eigenvalues
$a_i$ of $\A_{mm}$, and then compute $\st = \sum_i a_i/(a_i + 1)$. We also
recycle the eigenvalues to precompute $\log\det(\I + \Lbh) = \log\det(\I + \A_{mm}) = \sum_{i} \log(a_i + 1)$.
can finally precompute $\alpha$ and $q$.

\textbf{Phase 3: sampling loop}

Sampling $K$ and computing $C_K$ is immediate, and we can directly
use the probabilities $l_i$ to sample $\sigma$. Once we have $\sigma$,
we need to compute acceptance the acceptance probability (threshold),
which we do using logarithms for numerical precision, as follow
\begin{align*}
\frac{\det(\I+\Lbt_\sigma)}{C_K\det(\I+\Lbh)}
= \exp\left\{\log\det(\I+\Lbt_\sigma) - \log(C_K) - \log\det(\I+\Lbh)\right\},
\end{align*}
where we already have computed $\log\det(\I+\Lbh)$,
and $\log(C_K)$ is immediate.
Given $\W_{\sigma} = \diag(\sh l_i) \in \R^{K \times K}$
we have 
\begin{align*}
\log\det(\I + \Lbt_\sigma)
&= \log\det(\I + \W_{\sigma}^{-1/2}\L_\sigma \W_{\sigma}^{-1/2})
= \log\det(\W_{\sigma}^{-1/2}(\W_{\sigma} + \L_\sigma)\W_{\sigma}^{-1/2})\\
&= \log\det(\W_{\sigma}^{-1}) + \log\det(\W_{\sigma} + \L_\sigma)
= \sum_{i \in \sigma} -\log(\sh l_i) + \log\det(\W_{\sigma} + \L_\sigma)
\end{align*}

\textbf{Phase 4: DPP sampling}
Once we have $\Lbt_{\sigma}$, we simply feed it to \url{DPPy}'s
exact DPP sampler as a likelihood matrix, and sample.

